BaseMirror: Automatic Reverse Engineering of Baseband Commands from Android's Radio Interface Layer

In modern mobile devices, baseband is an integral component running on top of cellular processors to handle crucial radio communications. However, recent research reveals significant vulnerabilities in these basebands, posing serious security risks like remote code execution. Yet, effectively scrutinizing basebands remains a daunting task, as they run closed-source and proprietary software on vendor-specific chipsets. Existing analysis methods are limited by their dependence on manual processes and heuristic approaches, reducing their scalability. This paper introduces a novel approach to unveil security issues in basebands from a unique perspective: to uncover vendor-specific baseband commands from the Radio Interface Layer (RIL), a hardware abstraction layer interfacing with basebands. To demonstrate this concept, we have designed and developed BaseMirror, a static binary analysis tool to automatically reverse engineer baseband commands from vendor-specific RIL binaries. It utilizes a bidirectional taint analysis algorithm to adeptly identify baseband commands from an enhanced control flow graph enriched with reconstructed virtual function calls. Our methodology has been applied to 28 vendor RIL libraries, encompassing a wide range of Samsung Exynos smartphone models on the market. Remarkably, BaseMirror has uncovered 873 unique baseband commands undisclosed to the public. Based on these results, we develop an automated attack discovery framework to successfully derive and validate 8 zero-day vulnerabilities that trigger denial of cellular service and arbitrary file access on a Samsung Galaxy A53 device. These findings have been reported and confirmed by Samsung and a bug bounty was awarded to us.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> table/diffcmds.tex <==
\begin{table*}[t]
    \centering
     \scriptsize
    \begin{tabular}{lllll}
    \toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Write}} & \multicolumn{2}{c}{\textbf{Read}} \\ 
        ~ & BaseUni & CurUni & BaseUni & CurUni \\
        \midrule 
        A536 & / & / & / & / \\
        \midrule
        A205,A305,A405,A415 & \\
        A505,A606,A705,A805 & \\
        \midrule
        G981,G991,N981      & \texttt{A426-Write-BaseUni} &   &  \texttt{A426-Read-BaseUni}     & \texttt{A426-Read-TarUni} $\bigcup$  \\
                            &                             &   &                                 &  41JsonData::IpcRxGetPsiQueryInfo \\
        \midrule
        A426,A526,A725,A908 & 41JsonData::IpcTxGetQoSInfo & ~ & 41JsonCall::IpcRxCallExtEccList & 41Call::IpcRxBurstDtmf \\
                            &                             & ~ & 41JsonData::IpcRxQoSInfo        & 41Call::IpcRxCall*(16) \\ \bottomrule
    \end{tabular}
    \caption{Details of Discrepancy in Write and Read related commands between each firmware and the Baseline resident in \textit{Ipc41}(Upper) and \textit{Ipc41X}(Lower) seperately.}
    \label{tab:diffcmds}
\end{table*}
% {\S} for IpcProtocol40
% {\P} for IpcProtocol41
% for IpcProtoc



==> table/quantity.tex <==
\begin{table}[t]
  \centering
   \scriptsize
 % \scalebox{1.00}{
    \begin{tabular}{llrrrrr}
    \toprule
        \textbf{Protocol} & \textbf{Model} & \textbf{Vcall} & \textbf{Write} & \textbf{Read} & \textbf{Ioctl} & \textbf{Sendto} \\ \midrule
        \multirow{8}{*}{\textbf{Ipc41}} 
        & N975 & 2,828 & 478 & 49 & 41 & 2 \\ 
        ~ & J600 & 2,476 & 427 & 53 & 40 & 2 \\ 
        ~ & G920 & 3,057 & 570 & 67 & 45 & 1 \\ 
        ~ & G930 & 2,736 & 433 & 53 & 45 & 2 \\ 
        ~ & G960 & 3,020 & 493 & 55 & 44 & 2 \\ 
        ~ & G950 & 2,552 & 445 & 53 & 37 & 2 \\ 
        ~ & N950 & 2,551 & 429 & 53 & 39 & 2 \\ 
        ~ & N960 & 3,517 & 493 & 55 & 62 & 2 \\ \midrule
        \multirow{20}{*}{\textbf{Ipc41X}} 
        & A205 & 3,300 & 505 & 204 & 42 & 2 \\ 
        ~ & A305 & 3,301 & 505 & 204 & 42 & 2 \\ 
        ~ & A405 & 3,302 & 505 & 204 & 42 & 2 \\ 
        ~ & A415 & 3,296 & 505 & 204 & 45 & 2 \\ 
        ~ & A505 & 3,304 & 505 & 204 & 42 & 2 \\ 
        ~ & A606 & 4,549 & 505 & 204 & 59 & 2 \\ 
        ~ & A705 & 4,550 & 505 & 204 & 59 & 2 \\ 
        ~ & A805 & 4,549 & 505 & 204 & 59 & 2 \\ 
        ~ & G981 & 3,327 & 525 & 205 & 42 & 2 \\ 
        ~ & G991 & 3,327 & 525 & 205 & 42 & 2 \\ 
        ~ & N981 & 3,327 & 525 & 205 & 42 & 2 \\ 
        ~ & A426 & 4,580 & 525 & 204 & 59 & 2 \\ 
        ~ & A526 & 4,580 & 525 & 204 & 59 & 2 \\ 
        ~ & A725 & 4,580 & 525 & 204 & 59 & 2 \\ 
        ~ & A908 & 4,578 & 525 & 204 & 59 & 2 \\ 
        ~ & A515 & 3,323 & 526 & 189 & 36 & 2 \\ 
        ~ & A516 & 3,323 & 526 & 189 & 36 & 2 \\ 
        ~ & G973 & 3,320 & 526 & 189 & 36 & 2 \\ 
        ~ & G977 & 3,325 & 526 & 189 & 36 & 2 \\ 
        ~ & A536 & 3,327 & 526 & 189 & 36 & 2 \\ \bottomrule
    \end{tabular}
 % }
  \caption{Number of virtual calls and commands generated from each taint source per firmware.}
  \label{tab:allCmds}
\end{table}


==> table/statecheck.tex <==

\begin{algorithm}[t]
\caption{Baseband State Checking.}
\label{alg:statecheck}
\scriptsize
\SetAlgoLined
\DontPrintSemicolon
\newcommand\mycommfont[1]{\scriptsize\ttfamily\textcolor{black}{#1}}
\SetCommentSty{mycommfont}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
% \SetKwComment{Comment}{$\triangleright$\ }{}
\SetKwComment{Comment}{// }{}
\SetKwProg{Fn}{Function}{}{}
% \Input{$F$: \texttt{qt\_metacall} for class $c$, \texttt{index}: the property index}
% \Output{$ADDR$: the symbol address of property at \texttt{index} in $c$}
\Fn{\upshape state\_checking(cmd)} { \label{line:state_checking_init}
    send\_command(cmd)\;
    $s1 \leftarrow$ adb.exec("dumpsys telephony.registry")
    \Comment*[r]{to get modem state}
    \If{\upshape OUT\_OF\_SERVICE in $s1$} { 
        sleep(TIME\_SLOT) \;
        $s2 \leftarrow$ adb.exec("dumpsys telephony.registry")\;
        \If{\upshape OUT\_OF\_SERVICE in $s2$} {
            exec("reboot")\;
            $s3 \leftarrow$ adb.exec("dumpsys telephony.registry")\;
            \If{\upshape OUT\_OF\_SERVICE in $s3$} {
                \Return PERMANENT\_CRASH \Comment*[r]{reflash needed}
            }
            \Else{
                \Return RECOVERABLE\_CRASH \Comment*[r]{recover after reboot}
            }
        }
        \Else{
            \Return TEMPORARY\_CRASH \Comment*[r]{immediately crash after command}
        }
    }
    \Return NO\_CRASH \;
}
\end{algorithm}


